Optimizing error of high-dimensional statistical queries under differential privacy

Differentially private algorithms for answering sets of predicate counting queries on a sensitive database have many applications. Organizations that collect individual-level data, such as statistical agencies and medical institutions, use them to safely release summary tabulations. However, existing techniques are accurate only on a narrow class of query workloads, or are extremely slow, especially when analyzing more than one or two dimensions of the data. In this work we propose HDMM, a new differentially private algorithm for answering a workload of predicate counting queries, that is especially effective for higher-dimensional datasets. HDMM represents query workloads using an implicit matrix representation and exploits this compact representation to efficiently search (a subset of) the space of differentially private algorithms for one that answers the input query workload with high accuracy. We empirically show that HDMM can efficiently answer queries with lower error than state-of-the-art techniques on a variety of low and high dimensional datasets.

==> code.tex <==

\section{Pseudo Code}

\begin{algorithm}
\caption{\label{alg:ipinv} Implicit Pseudo Inverse}
{\small 
\begin{algorithmic}[1]
\Procedure{ImplicitPinv}{$B$}
\State $p,n = $ \Call{shape}{$B$}
\State $D^{-1} = $ \Call{diag}{\Call{ones}{$1$,$p$} $B$} 
\State $D = $ \Call{inv}{$D^{-1}$} 
\State $M = $ \Call{inv}{$I_p + B B^T$}
\Procedure{Dot}{$y$} \Comment $A^+ y = (A^T A)^{-1} A^T y$
\State $ y = \begin{bmatrix} y^{(1)} \\ y^{(2)} \end{bmatrix} $
\State $ u = D (y^{(1)} + B^T y^{(2)})$ \Comment $ A^T y $
\State \Return $ D^{-1} D^{-1} u - D^{-1} B^T (M (B D^{-1} u)) $  \Comment $ (A^T A)^{-1} a $
\EndProcedure

\Procedure{RDot}{$x$} \Comment $ (A^+)^T x = A (A^T A)^{-1} x $
\State $ u = D^{-1} D^{-1} x - D^{-1} B^T (M (B D^{-1} x)) $
\State \Return $ \begin{bmatrix} D u \\ B D u \end{bmatrix} $
\EndProcedure
\State \Return \Call{ImplicitMatrix}{Dot, RDot}
\EndProcedure
\end{algorithmic}}
\end{algorithm}

\begin{algorithm}
\caption{\label{alg:ikron} Implicit Kronecker Products}
{\small 
\begin{algorithmic}[1]
\Procedure{ImplicitKron}{$A$, $B$}
\State $ m_1, n_1 = $ \Call{shape}{$A$} 
\State $ m_2, n_2 = $ \Call{shape}{$B$}
\Procedure{Dot}{$x$}
\State $ X = $ \Call{mat}{$x$, $n_1 \times n_2$}
\State \Return \Call{vec}{$A X B^T$}
\EndProcedure

\Procedure{RDot}{$y$}
\State $ Y = $ \Call{mat}{$y$, $m_1 \times m_2$}
\State \Return \Call{vec}{$A^T Y B$}
\EndProcedure
\State \Return \Call{ImplicitMatrix}{Dot, RDot}
\EndProcedure
\item[]
\Procedure{Implicit Krons}{$A_1, \dots, A_d$}
\State \Return \Call{fold}{ImplicitKron, [$A_1, \dots, A_d$]}
\EndProcedure
\end{algorithmic}}
\end{algorithm}

\begin{algorithm}
\caption{\label{alg:ikrons} Implicit Kronecker Pseudo Inverse}
{\small 
\begin{algorithmic}[1]
\Procedure{Implicit Krons}{$B_1, \dots, B_d$}
\For{$i = 1, \dots d$}
\State $A_i^+ = $ \Call{ImplicitPinv}{$B_i$}
\EndFor
\State \Return \Call{Implicit Krons}{$A_1^+, \dots, A_d^+$}
\EndProcedure
\end{algorithmic}}
\end{algorithm}


==> kron.tex <==
\section{Representing high-dimensional workloads}  \label{sec:hd-workloads}

\gm{this section needs to be revised and augmented.  It should give the reader an accessible overview of the kinds of workloads we're interested in.  And then map between queries/workloads and vectors/matrices.  These are not central contributions, but the implicit representations are the main ``trick'' that enables scalability.}




\subsection{Definitions and Identities}

For multi-dimensional data, the cell condition $ \phi_i $ is usually a conjunction of cell conditions on each attribute.  With this in mind, it is sometimes convenient to organize the data into a matrix instead of a vector.  This enables us to reason about a special class of query matrices which will become important later. 

\begin{definition}[Vec]
For a matrix $\X$ where $ \x_1, \dots, \x_n $ are the rows of $\X$, $vec(\X)$ flattens $\X$ into a column vector in row-major order.  That is, $ vec(\X) = \begin{bmatrix} \x_1 & \dots & \x_n \end{bmatrix}^T $.
\end{definition}

\ry{explain why we need two sets of attributes}
\begin{definition}[Data Matrix]
For cell conditions $ \phi_i^{\mathbb{A}} $ and $ \phi_j^{\mathbb{B}} $ defined over disjoint sets of attributes $ \mathbb{A} $ and $ \mathbb{B} $ respectively, the data matrix $\X$ is a matrix where $ X_{ij} = | \set{t \in D \mid \phi_i^{\mathbb{A}}(t), \phi_j^{\mathbb{B}}(t)} | $.  The corresponding data vector is $ \x = vec(\X) $, and the element of $x_k$ corresponding to $X_{ij}$ has cell condition $ \phi_k^{\mathbb{A} \mathbb{B}} = \phi_i^{\mathbb{A}} \wedge \phi_j^{\mathbb{B}} $.
\end{definition}

This data matrix is nothing more than an intermediate representation that is useful to the discussion that follows.  It's easy to go back and forth between the two representations by flattening and reshaping the data.  We will sometimes refer to $ mat $ as the inverse operation of $vec$, which turns a data vector into a data matrix where the shape is implied by the context.  It's also possible to generalize the data matrix and organize $d$-dimensional data as a rank-$d$ tensor, although doing so is not necessary for the discussion that follows.

\begin{definition}[Query Intersection]
For queries $\vect{a}$ and $\vect{b}$ defined over disjoint sets of attributes $\mathbb{A}$ and $\mathbb{B}$, a data matrix $\X$ and an associated data vector $vec(\X)$, the query intersection $\vect{a} \sim \vect{b}$ maps two linear queries defined over $ \mathbb{A} $ and $ \mathbb{B} $ into a linear query defined over $ \mathbb{A} \cup \mathbb{B} $ such that
$$ (\vect{a} \sim \vect{b}) vec(\X) = \sum_{i,j} a_i b_j X_{ij} $$
which can be computed compactly as $ \vect{a} \X \vect{b}^T $.   
\end{definition}

If $\vect{a}$ and $\vect{b}$ both represent predicate counting queries, then $ \vect{a} \sim \vect{b} $ also represents a predicate counting query that counts how many tuples in the database satisfy the predicates from both $\vect{a}$ and $\vect{b}$.  Of course, this notion of query intersection generalizes to all linear counting queries, not just predicate counting queries. Nevertheless, it gives us a nice way to think about the operation.  

\begin{definition}[Cartesian Product in Query Space]
For query matrices $\A$ and $\B$ defined over disjoint sets of attributes $\mathbb{A}$ and $\mathbb{B}$, the cartesian product in query space, denoted $ \A \otimes \B $ contains the query intersection of every pair of queries from $\A$ and $\B$
\end{definition}

We'll now introduce the Kronecker product for matrices, as it is useful for computing the cartesian product in query space.

\begin{definition}[Kronecker products for matrices]
For two matrices $\A \in \mathbb{R}^{m \times n} $ and $\B \in \mathbb{R}^{m' \times n'}$, $ \A \otimes \B \in \mathbb{R}^{m \cdot m' \times n \cdot n'} $ where:

$$ \A \otimes \B = 
\begin{bmatrix}
a_{11} \B & \cdots & a_{1n} \B \\
\vdots & \ddots & \vdots \\
a_{m1} \B & \cdots & a_{mn} \B \\
\end{bmatrix}
$$
\end{definition}

Kronecker products satisfy the following identities:

\begin{enumerate}
\itemsep 0em
\item Associativity: $ (\A \otimes \B) \otimes \C = \A \otimes (\B \otimes \C) $
\item Mixed Product Property: $ (\A \otimes \B)(\C \otimes \D) = (\A \C) \otimes (\B \D) $
\item Pseudo Inverse: $ (\A \otimes \B)^+ = \A^+ \otimes \B^+ $
\item Matrix Equations: $ (\A \otimes \B) vec(\X) = vec(\A \X \B^T) $
\end{enumerate}

Proposition~\ref{prop:kron} shows that the cartesian product in query space can be computed with the Kronecker product.  

\begin{proposition} \label{prop:kron}
The cartesian product in query space between $\A$ and $\B$ can be obtained by computing the Kronecker product between $\A$ and $\B$.  
\end{proposition}

\begin{proof}
Let $\X$ be the data matrix and $ vec(\X) $ be the associated data vector.  Note that $ \A \X \B^T $ represents the answers to the desired set of queries, since $ (A X B^T)_{ij} = \vect{a}_i \X \vect{b}_j^T $, which is the query intersection between $\vect{a}_i$ and $\vect{b}_j$.  Using the matrix equations identity, we see that $ (\A \otimes \B) vec(\X) = vec(\A \X \B^T) $, so $ \A \otimes \B$ represents the desired set of queries for the data vector $ vec(\X) $, where $ \otimes $ is the Kronecker product.  
\end{proof}

It's easy to extend the results to show that query matrices can be constructed from the kronecker product of more than two matrices.  This is done by inductively applying proposition~\ref{prop:kron} with new query matrices.  For example, we could apply the proposition to show that the cartesian product in query space between $(\A \otimes \B) $ and $ \C $ is $ (\A \otimes \B) \otimes \C $.  Since $ \otimes $ is associative, the order that we arrange the parentheses doesn't matter and we can just write the query matrix as $ \A \otimes \B \otimes \C $.  A common case is to have one sub query matrix per attribute so that $ \A_i $ is the query matrix for the set of attributes $ \set{\mathcal{A_i}} $.   

\gm{moved this theorem here from later section}


These definitions give us a natural and compact way to represent many important high-dimensional workloads. 



==> related.tex <==
\section{Related Work} \label{sec:related}

Much research has been done to develop differenentially private algorithms for accurately answering linear queries.  See~\cite{hay2016principled} for a good overview of the state of the art.  These algorithms are either data-dependent (such as DAWA~\cite{li2014data}) or data-independent (such as $\matr{H}_b$~\cite{qardaji2013understanding}).  Hay et al. found that in the high signal setting (number of tuples is large relative to $\epsilon$ and $N$), data-independent algorithms dominate, while in the low signal setting, data-dependent algorithms dominate~\cite{hay2016principled}. 

Most of the data-independent use the \textbf{select-measure-reconstruct} paradigm, and much research has been done on the strategy selection problem for particular (usually fixed) workloads such as range queries or marginals.  Some research has been done on the strategy selection problem that is automatically tuned to a user-specified workload.  However, all existing approaches leave something to be desired in terms of scalability, generality, or utility. 

\subsubsection*{Range Queries}

One notable class of workloads that has recieved considerable attention in the literature is range queries.  For these workloads, Xiao et al. propose a strategy based on Wavelet transforms~\cite{xiao2011differential}, Hay et al. propose a hierarchical strategy~\cite{hay2010boosting}, Cormode et al propose similar hierarchical strategies for multi-dimensional domaains~\cite{cormode2012differentially}, and Qardaji et al. generalize and improve the hierarchical approach~\cite{qardaji2013understanding}.  All of these strategies are designed for workloads of range queries, and they are not workload-adaptive.  The $H_b$ approach proposed by Qardaji et al. chooses a branching factor for a hierarchical strategy by optimizing an analytically computable approximation of $ Error_{\R}(\matr{H}_b) $ where $\matr{H}_b$ is a hierarchical strategy.  Li et al. propose an approach called GreedyH~\cite{li2014data} that is workload adaptive, but based on a template strategy designed for range query-like workloads.  GreedyH can be seen as an instance of \sys, since it optimizes over strategies parameterized by a small set of weights, but the parameterization is only reasonable for 1D range query workloads, and is not expressive enough to capture the strategies produced by the General purpose parameterization we propose.

\subsubsection*{Marginals}

Another notable class of workloads that has recieved special attention in the literature is marginals.  Barak et al. propose a strategy based on Fourier basis vectors~\cite{barak2007privacy} for answering low-dimensional marginals over a binary domain.  This method offers some workload adaptivity, in that the set of Fourier basis vectors in the strategy depends on the marginals in the workload.  

Ding et al propose a strategy of marginals that adapts to the workload through a greedy heuristic~\cite{ding2011differentially} that approximately solves a combinatoric optimization problem.  This space of strategies considered by this approach is a subset of those representable by the marginals parameterization, where $ \vect{\theta} \in \set{0,1}^{2^d} $.  They give a method for efficiently doing least squares estimation for consistency, but their objective function doesn't account for this in the strategy selection phase. 

Qardaji et al. also propose a strategy of marginals that adapts to a workload through the solution to an optimization problem~\cite{qardaji2014priview}, but they don't require that the strategy support the workload.  They approximate the answers to unsupported queries by doing maximum entropy estimation.  One benefit of this approach is that many fewer queries need to be asked, which in turns lowers the sensitivity and consequently the noise per query answer.  However, this causes the many query answers to be biased, with the bias increasing with the amount of signal in the data.  

\subsubsection*{Adaptive}

Some existing methods are truly workload-adaptive.  Yuan et al. propose the low rank mechanism~\cite{yuan2012low} which finds strategies that do not fully support the workload and therefore produce biased query answers; while general, it fails to consistently outperform heuristic methods like \cite{xiao2011differential, hay2010boosting,qardaji2013differentially} on range query workloads. 

%Some workload-adaptive strategies have been proposed as well.  For example, in Li et al. show that solving a rank constrained semidefinite program leads to a globally optimal strategy~\cite{li2010optimizing}.  However, they did not have a practical algorithm for solving this difficult problem.  In~\cite{li2012adaptive}, Li et al. proposed the adaptive mechanism, which approximately solves the optimizing problem by restricting the search space to a row reweighting of some template strategy, where the default template strategy is based on the eigendecomposition of $ \W^T \W $.  The mechanism can be seen as an instance of PMM and while this approach offers reasonable scalability and works well for $(\epsilon, \delta)$-differential privacy, it does not provide acceptable utility in the $\epsilon$-differential privacy regime. 


%targets $\epsilon$-differential privacy and solves the problem by finding a workload decomposition $ \W \approx \B \L $.  Within the matrix mechanism framework, we can think of $ \L = \A $ and $ \B = \W \A^+ $.  In solving the optimization problem, they ignore the constraint that $\A$ supports $\W$ and instead only require that $ || \W \A^+ \A - \W || \leq \gamma $.  Due to this relaxation, the estimated workload query answers under this mechanism are biased, and the amount of bias increases with the amount of data available.  Furthermore, even though the approach is general in principle, it failed to consistently offer lower error than the static strategies for range query workloads.

% Their method is general (works for any workload), scalable (up to $n = 8192$), and provides optimal utility.  However, it only solves the optimization problem for $(\epsilon, \delta)$-differential privacy, and the method does not generalize to $\epsilon$-differential privacy.  This method can be used as a drop-in replacement for the general purpose mechanism in the $(\epsilon, \delta)$-differential privacy regime.  

